Compensating Supervision Incompleteness with Prior Knowledge in Semantic Image Interpretation

Semantic Image Interpretation is the task of extracting a structured semantic description from images. This requires the detection of visual relationships: triples (subject,relation,object) describing a semantic relation between a subject and an object. A pure supervised approach to visual relationship detection requires a complete and balanced training set for all the possible combinations of (subject, relation, object). However, such training sets are not available and would require a prohibitive human effort. This implies the ability of predicting triples which do not appear in the training set. This problem is called zero-shot learning. State-of-the-art approaches to zero-shot learning exploit similarities among relationships in the training set or external linguistic knowledge. In this paper, we perform zero-shot learning by using Logic Tensor Networks, a novel Statistical Relational Learning framework that exploits both the similarities with other seen relationships and background knowledge, expressed with logical constraints between subjects, relations and objects. The experiments on the Visual Relationship Dataset show that the use of logical constraints outperforms the current methods. This implies that background knowledge can be used to alleviate the incompleteness of training sets.

==> bibliovrd.tex <==
@inproceedings{Zellers18motifs,
  author    = {Rowan Zellers and
               Mark Yatskar and
               Sam Thomson and
               Yejin Choi},
  title     = {Neural Motifs: Scene Graph Parsing With Global Context},
  booktitle = {{CVPR}},
  pages     = {5831--5840},
  publisher = {{IEEE} Computer Society},
  year      = {2018}
}

@inproceedings{Larochelle2008Zero,
  author    = {Hugo Larochelle and
               Dumitru Erhan and
               Yoshua Bengio},
  title     = {Zero-data Learning of New Tasks},
  booktitle = {{AAAI}},
  pages     = {646--651},
  publisher = {{AAAI} Press},
  year      = {2008}
}

@inproceedings{biggio12poisoning,
  author    = {Battista Biggio and
               Blaine Nelson and
               Pavel Laskov},
  title     = {Poisoning Attacks against Support Vector Machines},
  booktitle = {{ICML}},
  publisher = {icml.cc / Omnipress},
  year      = {2012}
}

@INPROCEEDINGS {Serafini2016ltn,
  author    = {Luciano Serafini and
               Artur S. d'Avila Garcez},
  title     = {Learning and Reasoning with Logic Tensor Networks},
  booktitle = {AI*IA},
  series    = {LNCS},
  volume    = {10037},
  pages     = {334--348},
  publisher = {Springer},
  year      = {2016}
}

@article{Lampert2014Attribute,
  author    = {Christoph H. Lampert and
               Hannes Nickisch and
               Stefan Harmeling},
  title     = {Attribute-Based Classification for Zero-Shot Visual Object Categorization},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {36},
  number    = {3},
  pages     = {453--465},
  year      = {2014}
}

@inproceedings{Plummer2017phrase,
  author    = {Bryan A. Plummer and
               Arun Mallya and
               Christopher M. Cervantes and
               Julia Hockenmaier and
               Svetlana Lazebnik},
  title     = {Phrase Localization and Visual Relationship Detection with Comprehensive
               Image-Language Cues},
  booktitle = {{ICCV}},
  pages     = {1946--1955},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@ARTICLE {yin2018zoom,
  title={Zoom-Net: Mining Deep Feature Interactions for Visual Relationship Recognition},
  author={Yin, Guojun and Sheng, Lu and Liu, Bin and Yu, Nenghai and Wang, Xiaogang and Shao, Jing and Loy, Chen Change},
  journal={arXiv preprint arXiv:1807.04979},
  year={2018}
}

@INPROCEEDINGS {ramanathan2015learning,
  author    = {Vignesh Ramanathan and
               Congcong Li and
               Jia Deng and
               Wei Han and
               Zhen Li and
               Kunlong Gu and
               Yang Song and
               Samy Bengio and
               Chuck Rosenberg and
               Fei{-}Fei Li},
  title     = {Learning semantic relationships for better action retrieval in images},
  booktitle = {{CVPR}},
  pages     = {1100--1109},
  publisher = {{IEEE} Computer Society},
  year      = {2015}
}

@BOOK {hajek2001metamathematics,
    author    = "H{\'a}jek, P.",
    title     = "Metamathematics of Fuzzy Logic",
    publisher = "Springer",
    year      = "2001",
    series    = "Trends in Logic",
    isbn      = "9781402003707",
    lccn      = "98030404",
    url       = "https://books.google.it/books?id=Eo-e8Pi-HmwC"
}

@ARTICLE {nickel2016Review,
  author    = {Maximilian Nickel and
               Kevin Murphy and
               Volker Tresp and
               Evgeniy Gabrilovich},
  title     = {A Review of Relational Machine Learning for Knowledge Graphs},
  journal   = {Proceedings of the {IEEE}},
  volume    = {104},
  number    = {1},
  pages     = {11--33},
  year      = {2016}
}

@ARTICLE {bloch2005fuzzySpatial,
  author    = {Isabelle Bloch},
  title     = {Fuzzy spatial relationships for image processing and interpretation:
               a review},
  journal   = {Image Vision Comput.},
  volume    = {23},
  number    = {2},
  pages     = {89--110},
  year      = {2005}
}

@ARTICLE {gupta2015visual,
    author  = "Gupta, Saurabh and Malik, Jitendra",
    title   = "Visual semantic role labeling",
    journal = "arXiv preprint arXiv:1505.04474",
    year    = "2015"
}

@INPROCEEDINGS {sadeghi2011recognition,
    author       = "Sadeghi, Mohammad Amin and Farhadi, Ali",
    title        = "Recognition using visual phrases",
    booktitle    = "{CVPR}",
    year         = "2011",
    pages        = "1745--1752",
    organization = "IEEE"
}

@ARTICLE {hudelot2008fuzzy,
  author    = {C{\'{e}}line Hudelot and
               Jamal Atif and
               Isabelle Bloch},
  title     = {Fuzzy spatial relation ontology for image interpretation},
  journal   = {Fuzzy Sets and Systems},
  volume    = {159},
  number    = {15},
  pages     = {1929--1951},
  year      = {2008}
}

@ARTICLE {Hudelot2014FCA,
  author    = {Jamal Atif and
               C{\'{e}}line Hudelot and
               Isabelle Bloch},
  title     = {Explanatory Reasoning for Image Understanding Using Formal Concept
               Analysis and Description Logics},
  journal   = {{IEEE} Trans. Systems, Man, and Cybernetics: Systems},
  volume    = {44},
  number    = {5},
  pages     = {552--570},
  year      = {2014}
}

@INPROCEEDINGS {Peraldi2009formalizing,
  author    = {Irma Sof{\'{\i}}a Espinosa Perald{\'{\i}} and
               Atila Kaya and
               Ralf M{\"{o}}ller},
  title     = {Formalizing Multimedia Interpretation based on Abduction over Description
               Logic Aboxes},
  booktitle = {Description Logics},
  series    = {{CEUR} Workshop Proceedings},
  volume    = {477},
  publisher = {CEUR-WS.org},
  year      = {2009}
}

@INPROCEEDINGS {chen2012understanding,
  author    = {Na Chen and
               Qian{-}Yi Zhou and
               Viktor K. Prasanna},
  title     = {Understanding web images by object relation network},
  booktitle = {{WWW}},
  pages     = {291--300},
  publisher = {{ACM}},
  year      = {2012}
}

@INPROCEEDINGS {chen14PascalPart,
  author    = {Xianjie Chen and
               Roozbeh Mottaghi and
               Xiaobai Liu and
               Sanja Fidler and
               Raquel Urtasun and
               Alan L. Yuille},
  title     = {Detect What You Can: Detecting and Representing Objects Using Holistic
               Models and Body Parts},
  booktitle = {{CVPR}},
  pages     = {1979--1986},
  publisher = {{IEEE} Computer Society},
  year      = {2014}
}

@INPROCEEDINGS {xu2017sceneGraph,
    author    = "Xu, Danfei and Zhu, Yuke and Choy, Christopher B. and Fei-Fei, Li",
    title     = "Scene Graph Generation by Iterative Message Passing",
    booktitle = "CVPR",
    year      = "2017",
    publisher = {{IEEE} Computer Society},
    month     = "July"
}

@INPROCEEDINGS {kulkarni2011baby,
  author    = {Girish Kulkarni and
               Visruth Premraj and
               Sagnik Dhar and
               Siming Li and
               Yejin Choi and
               Alexander C. Berg and
               Tamara L. Berg},
  title     = {Baby talk: Understanding and generating simple image descriptions},
  booktitle = {{CVPR}},
  pages     = {1601--1608},
  publisher = {{IEEE} Computer Society},
  year      = {2011}
}

@ARTICLE {krishna2016visualgenome,
  author    = {Ranjay Krishna and
               Yuke Zhu and
               Oliver Groth and
               Justin Johnson and
               Kenji Hata and
               Joshua Kravitz and
               Stephanie Chen and
               Yannis Kalantidis and
               Li{-}Jia Li and
               David A. Shamma and
               Michael S. Bernstein and
               Li Fei{-}Fei},
  title     = {Visual Genome: Connecting Language and Vision Using Crowdsourced Dense
               Image Annotations},
  journal   = {International Journal of Computer Vision},
  volume    = {123},
  number    = {1},
  pages     = {32--73},
  year      = {2017}
}

@inproceedings{serafini2017learning,
  author    = {Luciano Serafini and
               Ivan Donadello and
               Artur S. d'Avila Garcez},
  title     = {Learning and reasoning in logic tensor networks: theory and application
               to semantic image interpretation},
  booktitle = {{SAC}},
  pages     = {125--130},
  publisher = {{ACM}},
  year      = {2017}
}

@PHDTHESIS {Schuler2005verbnet,
    author    = "Schuler, Karin Kipper",
    title     = "Verbnet: A Broad-coverage, Comprehensive Verb Lexicon",
    school    = "University of Pennsylvania",
    year      = "2005",
    address   = "Philadelphia, PA, USA",
    note      = "AAI3179808",
    isbn      = "0-542-20049-X",
    publisher = "University of Pennsylvania"
}

@INPROCEEDINGS {Baker1998framenet,
 author    = {Collin F. Baker and
               Charles J. Fillmore and
               John B. Lowe},
  title     = {The Berkeley FrameNet Project},
  booktitle = {{COLING-ACL}},
  pages     = {86--90},
  publisher = {Morgan Kaufmann Publishers / {ACL}},
  year      = {1998}
}

@inproceedings{donadello2017ijcai,
  author    = {Ivan Donadello and
               Luciano Serafini and
               Artur S. d'Avila Garcez},
  title     = {Logic Tensor Networks for Semantic Image Interpretation},
  booktitle = {{IJCAI}},
  pages     = {1596--1602},
  publisher = {ijcai.org},
  year      = {2017}
}

@inproceedings{Zhuang2017context,
  author    = {Bohan Zhuang and
               Lingqiao Liu and
               Chunhua Shen and
               Ian D. Reid},
  title     = {Towards Context-Aware Interaction Recognition for Visual Relationship
               Detection},
  booktitle = {{ICCV}},
  pages     = {589--598},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@inproceedings{Liang2017Deep,
  author    = {Xiaodan Liang and
               Lisa Lee and
               Eric P. Xing},
  title     = {Deep Variation-Structured Reinforcement Learning for Visual Relationship
               and Attribute Detection},
  booktitle = {{CVPR}},
  pages     = {4408--4417},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@inproceedings{Dai2017Detecting,
  author    = {Bo Dai and
               Yuqi Zhang and
               Dahua Lin},
  title     = {Detecting Visual Relationships with Deep Relational Networks},
  booktitle = {{CVPR}},
  pages     = {3298--3308},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@INPROCEEDINGS {tresp2017improvingVRD,
  author    = {Stephan Baier and
               Yunpu Ma and
               Volker Tresp},
  title     = {Improving Visual Relationship Detection Using Semantic Modeling of
               Scene Descriptions},
  booktitle = {ISWC {(1)}},
  pages     = {53--68},
  publisher = {Springer},
  year      = {2017}
}

@INPROCEEDINGS {lu2016visual,
  author    = {Cewu Lu and
               Ranjay Krishna and
               Michael S. Bernstein and
               Fei{-}Fei Li},
  title     = {Visual Relationship Detection with Language Priors},
  booktitle = {{ECCV} {(1)}},
  series    = {LNCS},
  volume    = {9905},
  pages     = {852--869},
  publisher = {Springer},
  year      = {2016}
}

@inproceedings{yu17vrd,
  author    = {Ruichi Yu and
               Ang Li and
               Vlad I. Morariu and
               Larry S. Davis},
  title     = {Visual Relationship Detection with Internal and External Linguistic
               Knowledge Distillation},
  booktitle = {{ICCV}},
  pages     = {1068--1076},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@inproceedings{Li2017ViP,
  author    = {Yikang Li and
               Wanli Ouyang and
               Xiaogang Wang and
               Xiaoou Tang},
  title     = {ViP-CNN: Visual Phrase Guided Convolutional Neural Network},
  booktitle = {{CVPR}},
  pages     = {7244--7253},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@inproceedings{Peyre2017Weakly,
  author    = {Julia Peyre and
               Ivan Laptev and
               Cordelia Schmid and
               Josef Sivic},
  title     = {Weakly-Supervised Learning of Visual Relations},
  booktitle = {{ICCV}},
  pages     = {5189--5198},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@inproceedings{Zhang2017VtransE,
  author    = {Hanwang Zhang and
               Zawlin Kyaw and
               Shih{-}Fu Chang and
               Tat{-}Seng Chua},
  title     = {Visual Translation Embedding Network for Visual Relation Detection},
  booktitle = {{CVPR}},
  pages     = {3107--3115},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@inproceedings{Zhang2017PPR-FCN,
  author    = {Hanwang Zhang and
               Zawlin Kyaw and
               Jinyang Yu and
               Shih{-}Fu Chang},
  title     = {{PPR-FCN:} Weakly Supervised Visual Relation Detection via Parallel
               Pairwise {R-FCN}},
  booktitle = {{ICCV}},
  pages     = {4243--4251},
  publisher = {{IEEE} Computer Society},
  year      = {2017}
}

@ARTICLE {neumann2008onscene,
    author    = "Bernd Neumann and               Ralf M{\"{o}}ller",
  title     = {On scene interpretation with description logics},
  journal   = {Image Vision Comput.},
  volume    = {26},
  number    = {1},
  pages     = {82--101},
  year      = {2008}
}

@inproceedings{donadello2014mixing,
  author    = {Ivan Donadello and
               Luciano Serafini},
  title     = {Mixing Low-Level and Semantic Features for Image Interpretation -
               {A} Framework and a Simple Case Study},
  booktitle = {{ECCV} Workshops {(2)}},
  series    = {Lecture Notes in Computer Science},
  volume    = {8926},
  pages     = {283--298},
  publisher = {Springer},
  year      = {2014}
}

@ARTICLE {donadello2016integration,
    author    = "Donadello, Ivan and Serafini, Luciano",
    title     = "Integration of numeric and symbolic information for semantic image interpretation",
    journal   = "Intelligenza Artificiale",
    year      = "2016",
    volume    = "10",
    number    = "1",
    pages     = "33--47",
    publisher = "IOS Press"
}
@inproceedings{donadello2015ontology,
  	author    = {Ivan Donadello},
  	title     = {Ontology Based Semantic Image Interpretation},
  	booktitle = {Proceedings of the Doctoral Consortium {(DC)} co-located with the 14th Conference of the Italian Association for Artificial Intelligence (AI*IA 2015), Ferrara, Italy, September 23-24, 2015.},
  	pages     = {19--24},
  	year      = {2015},
  	crossref  = {DBLP:conf/aiia/2015dc},
  	url       = {http://ceur-ws.org/Vol-1485/paper4.pdf},
  	timestamp = {Mon, 30 May 2016 16:28:37 +0200},
  	biburl    = {https://dblp.org/rec/bib/conf/aiia/Donadello15},
  	bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/aiia/2015dc,
  	editor    = {Elena Bellodi and Alessio Bonfietti},
  	title     = {Proceedings of the Doctoral Consortium {(DC)} co-located with the 14th Conference of the Italian Association for Artificial Intelligence (AI*IA 2015), Ferrara, Italy, September 23-24, 2015},
  	series    = {{CEUR} Workshop Proceedings},
  	volume    = {1485},
  	publisher = {CEUR-WS.org},
  	year      = {2015},
  	url       = {http://ceur-ws.org/Vol-1485},
  	urn       = {urn:nbn:de:0074-1485-8},
  	timestamp = {Mon, 30 May 2016 16:28:37 +0200},
  	biburl    = {https://dblp.org/rec/bib/conf/aiia/2015dc},
  	bibsource = {dblp computer science bibliography, https://dblp.org}
}
@BOOK {fellbaum98wordnet,
    title     = "{WordNet: an electronic lexical database}",
    publisher = "MIT Press",
    year      = "1998",
    added-at  = "2007-10-30T23:31:40.000+0100",
    biburl    = "http://www.bibsonomy.org/bibtex/2c9addc264aa2b922971d3d6e6c068cae/stumme",
    editor    = "Fellbaum, Christiane",
    interhash = "42daa1681607dd1d3f3234c605d84ec3",
    intrahash = "c9addc264aa2b922971d3d6e6c068cae",
    keywords  = "WordNet wordnet",
    timestamp = "2007-10-30T23:31:40.000+0100"
}

==> img/abstract.tex <==
\begin{abstract}
Semantic Image Interpretation is the task of extracting a structured semantic description from images. Such a task requires the detection of \emph{visual relationships}, i.e., triples \emph{$\langle$subject,~relation,~object$\rangle$} describing a semantic relation between a subject and an object. A pure supervised approach to visual relationship detection requires a complete and balanced training set for all the possible combinations of \emph{$\langle$subject,~relation,~object$\rangle$}. However, such a training set is not available and would require a prohibitive human effort. This implies that we should be able to predict triples which do not appear in the training set. This problem is called \emph{zero-shot learning}. State-of-the-art approaches to zero-shot learning exploit similarities among relationships in the training set 
or external linguistic knowledge. 
%
In this paper, we propose to use Logic Tensor Networks (LTNs), a novel Statistical Relational Learning framework that exploits both the similarities with other seen relationships and background knowledge, expressed in logical constraints between subjects, relations and objects. The experiments on the Visual Relationship Dataset show that the use of logical constraints in LTNs outperforms the current methods. This allows us to show that background knowledge can be used to alleviate the incompleteness of training sets. 
\end{abstract}

==> img/conclusions.tex <==
\section{Conclusions and Future Work}\label{sec:conclusions}
In this paper, we addressed the zero-shot learning in SII as the problem of detecting visual relationships whose instances do not appear in a training set. This is an emerging problem in AI datasets due to the high annotation effort and the consequent incompleteness of these datasets. Our proposal jointly exploits the similarity with other seen triples and some background knowledge. We used the framework Logic Tensor Networks that is suitable for this task as it is able to learn in presence of logical constraints. The results on the Visual Relationship Dataset show that the jointly use of data and logical constraints outperforms the state-of-the-art based on similarity with other triples or on linguistic statistical knowledge. This is due to the fact that logical constraints explicitly state the relations between a given relationship and its subject/object. The results allow us to state that logical knowledge compensates at the incompleteness of annotation in datasets. As future work, we plan to apply LTNs to the bigger Visual Genome dataset. We also want to study the performance by using different categories of constraints. In this manner, we check if there are constraints more effective than others.
\cleardoublepage

==> img/experiments.tex <==
\section{Experiments}\label{sec:evaluation}
\label{sec:results}
We conduct the experiments\footnote{The source code is available at \url{https://goo.gl/JgqYpu}.} on a dataset of visual relationships as the one described in the previous section. The dataset is the Visual Relationship Dataset (VRD) \cite{lu2016visual} that contains 4000 images for training and 1000 for testing annotated with visual relationships. Bounding boxes are annotated with a label in $\P_1$ containing 100 unary predicates. These labels refer to animals, vehicles, clothes and generic objects. Pairs of bounding boxes are annotated with a label in $\P_2$ containing 70 binary predicates. These label refer to actions, prepositions, spatial relations, comparatives or preposition phrases. The dataset has 37993 instances of visual relationships and 6672 types of relationships. 1877 instances of relationships occur only in the test set and they are used to evaluate the zero-shot scenario.

\paragraph{VRD Tasks} The performance of LTNs are tested on the following VRD standard tasks. The \textbf{phrase detection} is the prediction of a correct triple $\langle subject$, $predicate$, $object \rangle$ and its localization in a single bounding box containing both the subject and the object. The triple is a true positive if the labels are the same of the ground truth triple and if the predicted bounding box has at least 50\% of overlap with a corresponding bounding box in the ground truth. The ground truth bounding box is the union of the ground truth bounding boxes of the subject and of the object. The \textbf{relationship detection} task predicts a correct triple $\langle subject$, $predicate$, $object \rangle$ and the bounding boxes containing the subject and the object of the relationship. The triple is a true positive if both bounding boxes have at least 50\% of overlap with the corresponding ones in the ground truth. The labels for the predicted triple have to match with the ones of the corresponding triple in the ground truth. The \textbf{predicate detection} task predicts a set of correct binary predicates between a given set of bounding boxes. Here, the prediction does not depend on the performance of an object detector. The focus is only on the ability of LTNs to predict binary predicates.

\paragraph{Comparison} The performance of LTNs on these tasks have been evaluated with two LTNs grounded theories (or models): $\gtwo$ and $\gtw$. In the first one, $\gtwo = \langle \kwo, \pgsii \rangle$, $\kwo$ contains only positive and negative examples for the predicates in $\P$. This theory gives us the first results on the effectiveness of LTNs on visual relationship detection with respect to the state-of-the-art. In the second grounded theory $\gtw = \langle \kw, \pgsii \rangle$, $\kw$ contains examples and the logical constraints. With $\gtw$ we check the contribution of the logical constraints with respect to a standard machine learning approach. We first train the LTNs models on the VRD training set and then we evaluate them on the VRD test set. We evaluate all three tasks in a zero-shot learning scenario for testing the ability of LTNs to generalize to the 1877 relationships never seen in the training phase.

The LTNs models $\gtwo$ and $\gtw$ are compared with the following recent methods of the state-of-the-art \cite{lu2016visual,tresp2017improvingVRD,yu17vrd,Liang2017Deep,Zhuang2017context,Peyre2017Weakly,Zhang2017VtransE}. VRD \cite{lu2016visual} is the seminal work on visual relationship detection and provides the VRD. The method detects visual relationships by combining visual and semantic information. The visual information is the classification score given by two convolutional neural networks (CNNs). The first network classifies single bounding boxes according to the labels in $\P_1$. The second one classifies the union of two bounding boxes (subject and object) according to the labels in $\P_2$. These scores are combined with a language prior score (based on word embeddings) that models the semantics of the visual relationships. The methods in \cite{tresp2017improvingVRD} also combines visual and semantic information. However, link prediction methods (\emph{RESCAL}, \emph{MultiwayNN}, \emph{CompleEx}, \emph{DistMult}) are used for modelling the visual relationship semantics in place of word embeddings. In LKD \cite{yu17vrd} every visual relationship is predicted with a neural network trained on visual features and on the word embeddings of the subject/object labels. This network is regularized with a term that encodes statistical dependencies (taken from the training set and Wikipedia) between the predicates and subjects/objects. In VRL \cite{Liang2017Deep} the semantic information of the triples is modelled by building a graph of the visual relationships in the training set. A visual relationship is discovered (starting from the subject/object proposals coming from an object detector) with a graph traversal algorithm in a reinforcement learning setting. Context-AwareVRD \cite{Zhuang2017context} and WeaklySup \cite{Peyre2017Weakly} encode the features of pairs of bounding boxes similarly to Equation \eqref{eq:grCC}. However, in Context-AwareVRD the learning is performed with a neural network, whereas in WeaklySup the learning is based on a weakly-supervised discriminative clustering. That is, the supervision on a given relationship is not at triples level but on an image level. VTransE \cite{Zhang2017VtransE} uses only visual information of a CNN. Given the subject and object bounding boxes the binary predicate between them is predicted by learning the translation vector between the visual embeddings of the subject/object, i.e., $\mathbf{subj} + \mathbf{pred} \approx \mathbf{obj}$. 
\begin{table*}[ht]
\centering
\begin{tabular}{lcccccc}
\hline\hline
Task                                    	& Phrase Det. 	& Phrase Det. 	& Rel. Det. 	& Rel Det. 	& Pred. Det. 	& Pred. Det. 	\\ \hline
Evaluation                              	& R@100       	& R@50        	& R@100     	& R@50     	& R@100      	& R@50       	\\\hline\hline
VRD \cite{lu2016visual}                                                                                        & 3.75  & 3.36  & 3.52  & 3.13  & 8.45  & 8.45  \\
RESCAL \cite{tresp2017improvingVRD}                                                                                          & 6.59  & 5.82  & 6.07  & 5.3   & 16.34 & 16.34 \\
MultiwayNN \cite{tresp2017improvingVRD}                                                                                      & 6.93  & 5.73  & 6.24  & 5.22  & 16.6  & 16.6  \\
ComplEx \cite{tresp2017improvingVRD}                                                                                         & 6.5   & 5.73  & 5.82  & 5.05  & 15.74 & 15.74 \\
DistMult \cite{tresp2017improvingVRD} &4.19	&3.34	&3.85	&3.08	&12.4	&12.4\\
%$\gtwo$ (tesi)                                                                                        & 13.94 & 8.98  & 12.57 & 8.13  & 64.5  & 40.12 \\
%$\gtw$ (tesi)                                                                                        & 15.91 & 11.12 & 14.37 & 10.09 & 70.15 & 46.28 \\
$\gtwo$                                                                                               & 15.65 & 10.78 & 14.29 & 9.75  & 70.74 & 52.01 \\
$\gtw$                                                                                               & 16.51 & 12.23 & 15.23 & 11.29 & \textbf{76.65} & \textbf{55.95} \\
LKD \cite{yu17vrd}                                                                                       & \textbf{17.24} & \textbf{12.96} & \textbf{15.89} & \textbf{12.02} & 74.65 & 54.2  \\
%DRN \cite{Dai2017Detecting}                                    & -     & -     & -     & -     & -     & -     \\
VRL \cite{Liang2017Deep} & 10.31 & 9.17  & 8.52  & 7.94  & -     & -     \\
Context-AwareVRD \cite{Zhuang2017context}                  & 11.3  & 10.78 & 10.26 & 9.54  & 16.37 & 16.37 \\
%ViP-CNN \cite{Li2017ViP}                                      & -     & -     & -     & -     & -     & -     \\
WeaklySup \cite{Peyre2017Weakly}                                  & 7.8   & 6.8   & 7.4   & 6.4   & 21.6  & 21.6  \\
VTransE \cite{Zhang2017VtransE}                               & 3.51  & 2.65  & 2.14  & 1.71  & -     & -     \\
%PPR-FCN \cite{Zhang2017PPR-FCN}                  & -     & -     & -     & -     & -     & -     \\
%Zoom-Net (\underline{Arxiv})                    & -     & -     & -     & -     & -     & - \\
\hline\hline
\end{tabular}
\caption{Results on the Visual Relationship Dataset (R@K stands for recall at K). The use of the logical constraints in $\gtw$ leads to the best results and outperforms the state-of-the-art in the predicate detection task.}
\label{tb:vrd_results_zero}
\end{table*}

\paragraph{Evaluation Metric}
For each image in the test set, we use $\gtwo$ and $\gtw$ to compute the ranked set of groundings $\{\pgsii(\mathsf{r}(b,b'))\}_{\mathsf{r} \in \P_2}$, with $\langle b, b' \rangle$ bounding boxes computed with an object detector (the R-CNN model provided by \cite{lu2016visual}\footnote{\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}) or taken from the ground truth (for the predicate detection). We then perform the post processing. As evaluation metrics we use the \textbf{recall@100} and \textbf{recall@50} \cite{lu2016visual} as the annotation is not complete and precision would wrongly penalize true positives. We classify every pair $\langle b, b' \rangle$ of bounding boxes with \emph{all} the predicates in $\P_2$ as many relationships can occur between two objects (e.g., a person rides and is on a horse at the same time). and it is not possible to always define a preference notion between relationships. This choice is counterbalanced by predicting the the correct relationships within the top 100 and 50 positions.

%For each image in the test set, we use $\gtwo$ and $\gtw$ to compute the ranked set of groundings $\{\pgsii(\mathsf{r}(b,b'))\}_{\mathsf{r} \in \P_2}$, with $\langle b, b' \rangle$ bounding boxes computed with an object detector (the R-CNN model provided by \cite{lu2016visual}\footnote{\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}) or taken from the ground truth (for the predicate detection). In addition, every grounding $\pgsii(\mathsf{r}(b,b'))$ is multiplied with a prior: the frequency of the predicate $\mathsf{r}$ in the training set. As evaluation metrics we use the \textbf{recall@100} and \textbf{recall@50} \cite{lu2016visual} as the annotation is not complete and precision would wrongly penalize true positives. We classify every pair $\langle b, b' \rangle$ of bounding boxes with \emph{all} the predicates in $\P_2$ as many relationships can occur between two objects (e.g., a person rides and is on a horse at the same time). and it is not possible to always define a preference notion between relationships. This choice is counterbalanced by predicting the the correct relationships within the top 100 and 50 positions.

\paragraph{Implementation Details}
In Equations \eqref{eq:grUniv} and \eqref{eq:ltn_loss_sii} we set $p=-1$ (harmonic mean). The chosen t-norm is the \L{}ukasiewicz one. The number of tensor layers in Equation \eqref{eq:grP} is $k=5$ and $\lambda=10^{-10}$ in Equation \eqref{eq:ltn_loss_sii}. The optimization is performed separately on $\kw$ and $\kwo$ with 10000 training epochs of the RMSProp optimizer in \tensorflow.

\subsection{Discussion}
\label{sec:ltn_vrd_zero}
Table \ref{tb:vrd_results_zero} shows the results for the visual relationship detection tasks in the zero-shot learning scenario. The phrase and the relationship detection tasks are the hardest tasks, as they include also the detection of the bounding boxes of the subject/object. Therefore, the errors coming from the object detector propagate also to the visual relationship detection models. Adopting the same object detector used by VRD, \cite{tresp2017improvingVRD} and WeaklySup allows us to compare LTNs results starting from the same level of error coming from the bounding boxes detection. The $\gtwo$ and $\gtw$ models outperform these competitors showing that LTNs deal with the object detection errors in a better way. The predicate detection task, instead, is easier as it is independent from object detection. In this task, it is possible to see all the effectiveness of LTNs due to the good improvement of performance. Regarding the other competitors, a fully comparison is possible only in the predicate detection task as in the other tasks they use a different object detector for bounding boxes detection. However, both LTNs models effectively exploit the structure of the data to infer similarity between relationships and outperform VRL, Context-AwareVRD and VTransE. Moreover, the LTNs model $\gtw$ trained with data and constraints outperforms the model $\gtwo$ trained with only data. This means that the negative domain and range constraints are effective at excluding some binary predicates for a bounding box with a given subject or object. For example, if the subject is a physical object, then the predicate cannot be $\sleepOn$. This peculiarity of LTNs is fundamental in the comparison with LKD, as $\gtw$ achieves the improvement that outperforms LKD on predicate detection. The performance on the other tasks are comparable even if the data coming from the object detection are different. However, LKD exploits only statistical dependencies (co-occurrences) between subjects/objects and relationships, whereas LTNs exploit logical knowledge. This can express more information (e.g., positive or negative dependencies between subjects/objects and relationships, properties of the relationships, hierarchies of classes or relationships) and allows a more accurate reasoning on the visual relationships. Moreover, LKD has to predict $\mathcal{O}(|\P_1|^2|\P_2|)$ possible relationships, whereas the searching space of LTNs is $\mathcal{O}(|\P_1| + |\P_2|)$. This implies an important reduction of the parameters of the method and a substantial advantage on scalability.

These results prove two statements: (i) the general LTNs ability in the visual relationship detection problem to generalize to never seen relationships; (ii) the LTNs ability to leverage logical constraints in the background knowledge to improve the results in a zero-shot learning scenario. This important achievement states that it possible to use the logical constraints to compensate the lack of information in the datasets due to the effort of the annotation. These exploited logical constraints are not domain specific and can be retrieved from on-line linguistic resources.


%\subsection{Performance on a Normal Setting}
%\label{sec:ltn_vrd_perf}
%Table \ref{tb:vrd_results} shows the results for the visual relationships detection tasks. The first line presents the results in \cite{lu2016visual} and the following four lines the results in \cite{tresp2017improvingVRD} according to the link prediction models implemented. The last two lines show the LTNs results for $\gtwo$ and $\gtw$, respectively.
% \begin{table*}[htbp]
% \centering
% \begin{tabular}{lcccccc}
% \hline\hline 
% Task                                                                                            & Phrase Det. & Phrase Det. & Rel. Det. & Rel. Det. & Pred. Det. & Pred. Det. \\ \hline
% Evaluation                                                                                       & R@100            & R@50             & R@100          & R@50           & R@100               & R@50                \\\hline\hline
% VRD \cite{lu2016visual}                                                                                       & 17.03            & 16.17            & 14.7           & 13.86          & 47.87               & 47.87               \\
% RESCAL \cite{tresp2017improvingVRD}                                                                                          & 19.17            & 18.16            & 16.88          & 15.88          & 52.71               & 52.71               \\
% MultiwayNN \cite{tresp2017improvingVRD}                                                                                      & 18.88            & 17.75            & 16.65          & 15.57          & 51.82               & 51.82               \\
% ComplEx \cite{tresp2017improvingVRD}                                                                                         & 19.36            & 18.25            & 17.12          & 16.03          & 53.14               & 53.14               \\
% %$\gtwo$ (tesi)                                                                                        & 28.12            & 23.21            & 24.86          & 20.82          & 91.23               & 77.32               \\
% %$\gtw$ (tesi)                                                                                        & 28.24            & 22.72            & 25.1           & 20.63          & 91.88               & 78.63               \\
% NC                                                                                               & 26.87            & 22.96            & 23.71          & 20.58          & 91.02               & 81.29               \\
% WC                                                                                               & 26.15            & 22.02            & 23.2           & 19.8           & 91.61               & 81.11               \\
% LKD \cite{yu17vrd}                                                                                       & 29.43            & 26.32            & 31.89          & 22.68          & 94.65               & 85.64               \\
% DRN \cite{Dai2017Detecting}                                     & 23.45            & 19.93            & 20.88          & 17.73          & 81.9                & 80.78               \\
% VRL \cite{Liang2017Deep} & 22.6             & 21.37            & 20.79          & 18.19          & -                   & -                   \\
% Context-AwareVRD \cite{Zhuang2017context}                  & 25.56            & 24.04            & 23.52          & 20.35          & 53.59               & 53.59               \\
% ViP-CNN \cite{Li2017ViP}                                       & 27.91            & 22.78            & 20.01          & 17.32          & -                   & -                   \\
% \underline{WeaklySup} \cite{Peyre2017Weakly}                                  & 19.5             & 17.9             & 17.1           & 15.8           & 52.6                & 52.6                \\
% VTransE \cite{Zhang2017VtransE}                               & 22.42            & 19.42            & 15.2           & 14.07          & 44.76               & 44.76               \\
% PPR-FCN \cite{Zhang2017PPR-FCN}                  & 23.15            & 19.62            & 15.72          & 14.41          & 47.43               & 47.43               \\
% Zoom-Net (\underline{Arxiv})                    & 38.39            & 29.64            & 28.52          & 22.34          & 94.56               & 89.03   \\\hline\hline           
% \end{tabular}
% \caption[Results on the Visual Relationship Dataset]{Results on the Visual Relationship Dataset (R@K stands for recall at K). The $\gtwo$ and $\gtw$ models are comparable and always outperform the state-of-the-art.}
% \label{tb:vrd_results}
% \end{table*}
% The difficulty of this setting can be seen in the huge drop in performance for all the methods on all the tasks.
%The LTNs models outperform the original work on VRD \cite{lu2016visual} and the state-of-the-art \cite{tresp2017improvingVRD} on all the tasks for every measure. The phrase and the relationship detection tasks are the hardest, as they include also the detection of the bounding boxes of the subject and of the object. Therefore, the errors coming from the object detector propagate also to the visual relationship detection models. Adopting the same object detector used by our competitors allows us to compare LTNs results starting from the same level of error coming from the bounding boxes detection. The good results obtained by LTNs models show that LTNs deal with the object detection errors in a better way. The predicate detection task, instead, is easier as it is independent from object detection. We can see the improvement of performance on all the methods. In this task, it is possible to see all the effectiveness of LTNs due to the good improvement of performance. Indeed, the LTNs models are able to correctly classify more than the 90\% of all the given pairs of bounding boxes within the first 100 results. In this evaluation, the performance of $\gtwo$ and $\gtw$ are comparable. This fact suggests us that the negative domain and range constraints do not take particular effect on the optimization. Therefore, the improvement given by LTNs is mostly determined by the underlying Neural Tensor Network (Equation \ref{eq:grP}) and the encoding of the bounding boxes with semantic and (extra) geometric features.

==> img/intro.tex <==
\section{Introduction}\label{sec:intro}
Semantic Image Interpretation (SII) \cite{neumann2008onscene} concerns the automatic extraction of high-level information about the content of a visual scene. This information regards the objects in the scene, their attributes and the relations among them. Formally, SII extracts the so-called \emph{scene graph} \cite{krishna2016visualgenome} from a picture: the labelled nodes refer to objects in the scene and their attributes, the labelled edges regard the relations between the corresponding nodes. SII enables important applications on an image content that a coarser image analysis (e.g., the object detection) does not allow. For example, the \emph{visual question answering} (answering to natural language questions about the image content), the \emph{image captioning} (generating a natural language sentence describing the image content), the \emph{complex image querying} (retrieving images using structured queries about the image content) or the \emph{robot interaction} (different configurations of objects allow different actions for a robot). The visual relationship detection (VRD) is a special instance of scene graph construction. Indeed, a visual relationship is a triple $\langle subject, predicate, object \rangle$ where the subject and the object are the labels (or semantic classes) of two bounding boxes in the image. The predicate is the label regarding the relationship between the two bounding boxes. The construction of a scene graph from visual relationships is pretty forward. The subject and object are nodes in the graph with the corresponding labels, the predicate is a labelled edge from the subject node to the object node.

Visual relationships are mainly detected with supervised learning techniques \cite{yu17vrd}. These require large training sets of images annotated with bounding boxes and relationships \cite{lu2016visual,krishna2016visualgenome}. However, a complete and detailed annotation is not possible due to the high human effort of the annotators. For example, a person riding a horse can be annotated with the relations $\on$, $\ride$ (person subject) or $\below$, $\carry$ (horse subject). Thus, many types of relationships are not in the training set but can appear in the test set. The task of predicting visual relationships with never seen instances in the training phase is called \emph{zero-shot learning} \cite{Lampert2014Attribute}. This can be achieved by exploiting the similarity with the triples in the training set or using a high-level description of the relationship. For example, the fact that people ride elephants can be derived from a certain similarity between elephants and horses and the (known) fact that people can ride horses. This is closer to human learning with respect to supervised learning. Indeed, humans are able to both generalize from seen or similar examples and to use their background knowledge to identifying never seen relationships \cite{Lampert2014Attribute}. This background knowledge can be linguistic information about the subject/object and predicate occurrences \cite{lu2016visual,Zhang2017VtransE,yu17vrd} or logical constraints \cite{serafini2017learning,donadello2017ijcai}. Logical knowledge is very expressive and it allows us to explicitly state relations between subjects/objects and predicates. For example, the formula $\forall x,y( ride(x,y) \rightarrow elephant(y) \vee horse(y))$ states that the objects of the riding relations are elephants and horses. Other formulas can state that horses and elephants cannot ride and thus avoiding wrong predictions.

In this paper, we use Logic Tensor Networks (LTNs) \cite{Serafini2016ltn} for the detection of visual relationships. This is a Statistical Relational Learning framework specifically designed for learning from relational data (and exploiting the similarities with already seen triples) in presence of logical constraints. The results on the Visual Relationship Dataset show that the joint use of logical knowledge and data outperforms the state-of-the-art approaches based on data and/or linguistic knowledge. These promising results allow us to state that logical knowledge is able to counterbalance the lack of information in the datasets due to the high annotation effort.

==> img/ltn.tex <==
\section{Logic Tensor Networks}
\label{sec:ltn}
Logic Tensor Networks (LTNs) \cite{Serafini2016ltn} are a statistical relational learning framework that combine Neural Networks with logical constraints. LTNs adopt the syntax of a First-Order predicate language $\Lng$ whose signature is composed of two disjoint sets $\C$ and $\Pr$ denoting constants and predicate symbols, respectively. We do not present the LTNs framework for function symbols as they are not strictly necessary for the detection of visual relationships. For any predicate symbol $s$, let $\arity(s)$ denote its arity. $\Lng$ allows LTNs to express visual relationships and a priori knowledge about a domain. E.g., the visual relationship $\langle person, ride, horse\rangle$ is expressed with the atomic formulas $\person(p_1)$, $\horse(h_1)$ and $\ride(p_1, h_1)$. Common knowledge is expressed through logical constraints, e.g., $\forall x,y (\ride(x,y) \rightarrow \neg \dog(x))$ states that dogs do not ride.

LTNs semantics deviates from the \textit{abstract} semantics of Predicate Fuzzy Logic \cite{hajek2001metamathematics} towards a \textit{concrete} semantics. Indeed, the interpretation domain is a subset of $\mathbb{R}^n$, that is, constant symbols and closed terms are associated with a $n$-dimensional real vector. This vector encodes $n$ numerical features of an object. For example, the confidence score of an object detector for several classes of objects, the bounding box coordinates, the area, local features, etc. Predicate symbols are interpreted as functions on real vectors to the interval $[0,1]$. The interpretation of a formula represents the degree of truth for that formula: an higher value means a higher degree of truth. LTNs use the term \emph{grounding} (symbol $\G$) as synonym of logical interpretation in a ``real'' world. A grounding has to capture the latent correlation between the features of objects and their categorical/relational properties.
\begin{definition} 
An $n$-\emph{grounding} $\G$ (with $n \in\Nat$, $n > 0$), or simply \emph{grounding}, for a First-Order Language $\Lng$ is a function from the signature of $\Lng$ that satisfies the conditions:
\begin{enumerate}
\item $\G(c)\in\R^n$, for every $c\in\C$;
%\item $\G(f)\in \R^{n\cdot \arity(f)}\longrightarrow \R^n$ for every $f\in\Fn$;
\item $\G(P)\in \R^{n\cdot \arity(P)}\longrightarrow [0,1]$, for every $P\in\Pr$. 
\end{enumerate}
\end{definition}
\noindent Given a grounding $\G$ and let $\term(\Lng) = \{t_1, t_2, t_3, \ldots\}$ be the set of closed terms of $\Lng$, the semantics of atomic formulas is inductively defined as follows:
\begin{align}\label{eq:grPf}
%\G(f(t_1,\dots,t_m)) 		& = \G(f)(\G(t_1),\dots,\G(t_m)) \nonumber \\ 
\G(P(t_1,\dots,t_m)) 		& = \G(P)(\G(t_1),\dots,\G(t_m)).
\end{align}
\noindent The semantics for non-atomic formulas is defined according to t-norms functions used in Fuzzy Logic. If we take, for example, the \L{}ukasiewicz t-norm, we have:
\begin{align}
\label{eq:grLuk}
\G(\phi\imp\psi) 		& = \min(1,1-\G(\phi)+\G(\psi))			\nonumber\\
\G(\phi\wedge\psi) 		& = \max(0,\G(\phi)+\G(\psi) - 1) 		\nonumber\\ 
\G(\phi\vee\psi) 		& = \min(1,\G(\phi)+\G(\psi)) 			\nonumber\\ 
\G(\neg\phi) 			& = 1-\G(\phi).
\end{align}
\noindent
The semantics for quantifiers differs from the semantics of standard Fuzzy Logic. Indeed, the interpretation of $\forall$ leads the definition:
\begin{equation}
\G(\forall x \phi(x)) = \inf\{\G(\phi(t)) | t \in \term(\Lng)\}.
\end{equation}
This definition does not tolerate exceptions. E.g., the presence of a dog riding a horse in a circus would falsify the formula that dogs do not ride. LTNs handle these outliers giving a higher truth-value to the formula $\forall x \phi(x)$ if many examples satisfy $\phi(x)$. This is in the spirit of SII as in a picture (due to occlusions or unexpected situations) some common logical constraints are not always respected.
\begin{definition}
\label{def:grUniv}
Let $mean_p(x_1,\dots,x_d) = \left(\frac{1}{d}\sum_{i=1}^d x_i^{p}\right)^{\frac{1}{p}}$, with $p\footnote{The popular mean operators (arithmetic, geometric and harmonic mean) are obtained by setting p = 1, 2, and -1, respectively.} \in \mathbb{Z}$, $d \in \mathbb{N}$, the grounding for $\forall x \phi(x)$ is
\begin{multline}
\label{eq:grUniv}
\G(\forall x \phi(x)) = \\
\lim_{d\rightarrow \vert \term(\Lng) \vert }mean_p(\G(\phi(t_1)), \ldots ,\G(\phi(t_d))).
\end{multline}
\end{definition}
\noindent The grounding of a quantified formula $\forall x \phi(x)$ is the mean of the $d$ groundings of the quantifier-free formula $\phi(x)$.
%The semantics of $\exists$ is usually determined by exploiting the equivalence between $\exists$ and $\neg\forall\neg$. However, if we consider the Lukasiewicz t-norm and the arithmetic mean, we have that $\G(\forall x \phi(x))=\G(\exists x\phi(x))$. Therefore, in LTNs the existential quantification is interpreted via Skolemization: every formula of the form $\forall x_1,\dots,x_n(\dots \exists y \phi(x_1,\dots,x_n,y))$ is rewritten as $\forall x_1,\dots,x_n(\dots \phi(x_1,\dots,x_n,f(x_1,\dots,x_n)))$, with $f(x_1,\dots,x_n)$ a \emph{Skolem function}, that is a new $n$-ary function symbol.

A suitable function for a grounding should preserve some form of $\textit{regularity}$. Let us consider a constant $b \in \C$ that refers to a bounding box containing a horse. Let $\bv$ be the feature vector returned by the grounding of $b$, then it holds that $\G(\horse)(\bv)\approx 1$. Moreover, for every bounding box with feature vector $\bv'$ similar to $\bv$, $\G(\horse)(\bv')\approx 1$ holds. These functions are learnt from data\footnote{Some groundings can be manually defined with some rules \cite{donadello2017ijcai,bloch2005fuzzySpatial}. However, for some predicates this could be time consuming or inaccurate \cite{donadello2017ijcai}.} by tweaking their inner parameters in a training process that fits a training set. These functions are linear transformations or Neural Networks. 
%The grounding for \textbf{function symbols} is based on linear transformations from $\R^{mn}$ to $\R^{n}$. Let $b_1,\ldots,b_m \in \C$ with feature vectors $\bv_i = \G(b_i) \in \mathbb{R}^n$, with $i = 1 \ldots m$, and $\bv=\left<\bv_1;\dots;\bv_m\right>$ is a $mn$-ary vector given by the vertical stacking of each vector $\bv_i$. If $f$ is a $m$-ary function then:
%\begin{equation}
%\label{eq:grF}
%\G(f)(\bv)= M_f\bv + N_f.
%\end{equation}
%The parameters of $\G(f)$ are the $n\times mn$ real matrix $M_f$ and the $n$-vector $N_f$.
The grounding for \textbf{predicate symbols} is a generalization of a neural tensor network: an architecture proved to be effective at learning general relationships from similarities with other types of relationships \cite{nickel2016Review}. Let $b_1,\ldots,b_m \in \C$ with feature vectors $\bv_i = \G(b_i) \in \mathbb{R}^n$, with $i = 1 \ldots m$, and $\bv=\left<\bv_1;\dots;\bv_m\right>$ is a $mn$-ary vector given by the vertical stacking of each vector $\bv_i$. The grounding $\G(P)$ of an $m$-ary predicate $P(b_1,\ldots,b_m)$ is:
\begin{align}
\label{eq:grP}
\G(P)(\bv) = \sigma\left(u^\intercal_P\tanh\left(\bv^\intercal W_P^{[1:k]}\bv + V_P\bv + b_P\right)\right)
\end{align}
with $\sigma$ the sigmoid function. The parameters for $P$ are: $u_P \in \R^{k}$, a 3-D tensor $W_P^{[1:k]} \in \R^{k \times mn\times mn}$, $V_P \in \R^{k\times mn}$ and $b_P \in \R^{k}$. The parameter $u_P$ computes a linear combination of the quadratic features returned by the tensor product. With Equations \eqref{eq:grPf} and \eqref{eq:grP} the grounding of a complex LTNs formula can be computed by first computing the groundings of the closed terms and the atomic formulas contained in the complex formula. Then, these groundings are combined using a specific t-norm, see Equation \eqref{eq:grLuk}.

Learning the groundings involves the optimization of the truth values of the formulas in a LTNs knowledge base, a.k.a. \emph{grounded theory}. A \emph{partial grounding} $\pG$ is a grounding defined on a subset of the signature of $\Lng$. A grounding $\G$ for $\Lng$ is a \emph{completion} of $\pG$ (in symbols $\pG \subseteq \G$) if $\G$ coincides with $\pG$ on the symbols where $\pG$ is defined.

\begin{definition}%[Grounded Theory]
A \emph{grounded theory GT} is a pair $\GT$ with $\K$ a set of closed formulas and $\pG$ a partial grounding.
\end{definition}
\begin{definition}%[Satisfiability of a Grounded Theory]
A grounding $\G$ satisfies a grounded theory $\GT$ if $\pG \subseteq \G$ and $\G(\phi)=1$, for all $\phi\in\K$. A grounded theory $\GT$ is \emph{satisfiable} if there exists a grounding $\G$ that satisfies $\GT$. 
\end{definition}
\noindent According to the above definition, the satisfiability of $\GT$ can be obtained by searching for a grounding $\G$ that extends $\pG$ such that \emph{every} formula in $\K$ has value 1. When a grounded theory is not satisfiable a user can be interested in a degree of satisfaction of the GT.

\begin{definition}
Let $\GT$ be a grounded theory, the \emph{best satisfiability problem} amounts at searching an extension $\G^*$ of $\pG$ in $\GG$ (the set of all possible groundings) that maximizes the truth value of the conjunction of the formulas in $\K$:
\begin{equation}
\label{eq:besta}
\G^* = \argmax_{\pG \subseteq \G \in \GG}\G\left(\bigwedge_{\phi \in \K}\phi\right).
\end{equation}
\end{definition}

\noindent The best satisfiability problem is an optimization problem on the set of parameters to be learned. Let $\Theta = \{W_P,V_P,b_P,u_P \mid P\in\Pr\}$ be the set of parameters. Let $\G(\cdot|\Theta)$ be the grounding obtained by setting the parameters of the grounding functions to $\Theta$. The best satisfiability problem tries to find the best set of parameters $\Theta$:
\begin{equation}
\label{eq:ltn_loss}
\mbox{$\Theta^*=\argmax_{\Theta}\G\left(\left.\bigwedge_{\phi \in \K}\phi\right|\Theta\right) - \lambda\lVert\Theta\rVert_2^2$}
\end{equation}
with $\lambda\lVert\Theta\rVert_2^2$ a regularization term.

==> img/ltn_vrd.tex <==
\section{LTNs for Visual Relationship Detection}
Similarly to \cite{donadello2017ijcai}, we encode the problem of VRD with LTNs. However, the problem here is more challenging as a dataset for VRD contains many binary predicates and not only the $\partof$ as in \cite{donadello2017ijcai}.

Let $\pics$ be a VRD dataset with $B(p)$ its annotated set of bounding boxes for every picture $p \in \pics$. Each bounding box is annotated with a set of labels that describe the physical objects contained in the bounding boxes. Pairs of bounding boxes are annotated with the semantic relations between the contained physical objects. Let $\Sigma_{\text{SII}}=\left<\P,\C\right>$ be a $\Lng$ signature where $\Pr=\Pr_1 \cup \Pr_2$ is the set of predicates. $\Pr_1$ is the set of unary predicates that are the \emph{object types} (or \emph{semantic classes}) used to label the bounding boxes, e.g., $\Pr_1 = \{\horse, \person, \shirt,\pizza, \dots\}$. The set $\Pr_2$ contains binary predicates used to label pairs of bounding boxes, e.g., $\Pr_2 = \{\ride,\on,\wear, \eat, \dots\}$. Let $\C=\bigcup_{p\in\pics}B(p)$ be the set of constants for all the bounding boxes in the dataset $\pics$. However, the information in $\pics$ is incomplete: many bounding boxes (or pairs of) have no annotations or even some pictures have no annotations at all. Therefore, LTNs is used to exploit the information in $\pics$ to complete the missing information, i.e., to predict the visual relationships. As in \cite{donadello2017ijcai}, we encode $\pics$ with a grounded theory $\gtsii =\langle\ksii,\pgsii\rangle$ described in the following. The LTNs knowledge base $\ksii$ encodes the bounding box annotations in the dataset and some background knowledge about the domain. The task is to complete the partial knowledge in $\pics$ by finding a grounding $\G^*_\mathrm{SII}$, that extends $\pgsii$, such that:
$$
\begin{array}{lcl}
\G^*_\mathrm{SII}(C(b)) 			& \mapsto &	[0, 1]\\
\G^*_\mathrm{SII}(R(b_1, b_2)) 	& \mapsto &	[0, 1]
\end{array}
$$
for every unary ($C$) and binary ($R$) predicate symbol and for every (pair of) bounding box in the dataset.

\subsection{The Knowledge Base $\ksii$}
\label{sec:kb_sii}
The knowledge base $\ksii$ contains positive and negative examples (used for learning the grounding of the predicates in $\Pr$) and the background knowledge. The \textbf{positive examples} (taken from the annotations in $\pics$) for a semantic class $C$ are the atomic formulas $C(b)$, for every bounding box $b$ labelled with class $C \in \Pr_1$ in $\pics$. The positive examples for a relation $R$ are the atomic formulas $R(b_1, b_2)$, for every pair of bounding boxes $\left<b_1, b_2\right>$ labelled with the binary relation $R \in \Pr_2$ in $\pics$.

Regarding the \textbf{negative examples}, we differ from the \emph{Close World Assumption} (CWA) approach used in \cite{donadello2017ijcai}. CWA states that every unknown fact (that is, a missing label on a bounding box or pair of) is false and thus is a negative example. This holds for the dataset in \cite{chen14PascalPart} used in \cite{donadello2017ijcai} as it contains total information for the part-of relation. However, this does not hold for a general VRD dataset. Therefore, we adopt a relaxed version of the CWA. Regarding the negative examples for a semantic class $C$, we complete the annotations of the bounding boxes according to the IsA constraints of a knowledge base. E.g., the constraint $\forall x(\horse(x) \rightarrow \animal(x))$ will complete the annotation of the bounding boxes containing horses with the extra label ``animal''. The negative examples are then the atomic formulas $\neg C(b)$, for every bounding box $b$ not labelled with the class $C \in \Pr_1$. The negative examples for a relation $R$ are the atomic formulas $\neg R(b_1, b_2)$, for every pair of bounding boxes $\left<b_1, b_2\right>$ belonging to the same picture and not labelled with \emph{any} binary relation. Our approach avoids to consider, as negative examples for a relation $R$, bounding boxes annotated with another relation. E.g., if $b_1, b_2$ are annotated with only the $\ride$ relation, for the CWA $\langle b_1, b_2 \rangle$ is a (wrong) negative example for the $\on$ relation whereas our relaxed version avoids this issue.

Regarding the \textbf{background knowledge}, we manually build the logical constraints. We focus on the \emph{negative domain and range constraints} that list which are the semantic classes that cannot be the subject/object for a predicate. For example, clothes cannot drive. For every unary predicate $\dress$ in $\P_1$ that refers to a dress, the constraint $\forall xy(\drive(x,y) \imp \neg \dress(x))$ is added to $\mathcal{BK}$. In a large scale setting, these constraints can be retrieved by on-line linguistic resources such as FrameNet \cite{Baker1998framenet} and VerbNet \cite{Schuler2005verbnet} that provide the range and domain of binary relations through the so-called \emph{frames} data structure. Then, by applying mutual exclusivity between classes it is possible to derive the negative domain and range constraints. This class of constraints brings to good performance in the evaluation. A massive experimentation with other classes of constraints (such as IsA, mutual exclusivity, inverse, symmetry and reflexivity properties) is left as future work.

\subsection{The Grounding $\pgsii$}
As in \cite{donadello2017ijcai}, the grounding of each bounding box \textbf{constant} $b\in\C$ is a feature vector $\pgsii(b) = \bv_b \in \R^{|\Pr_1|+4}$ of \emph{semantic} and \emph{geometric} features:
\begin{multline}
\label{eq:grC}
\bv_b = \langle score(C_1,b),\dots,score(C_{|\Pr_1|},b)\\
x_0(b),y_0(b),x_1(b),y_1(b) \rangle,
\end{multline}
with $x_0(b),y_0(b),x_1(b),y_1(b)$ the coordinates of the top-left and bottom-right corners of $b$ and $score(C_i, b)$ is the classification score of an object detector for $b$ according to the class $C_i \in \Pr_1$. However, here we adopt the \emph{one-hot encoding}: the semantic features take value 1 in the position of the class with the highest detection score, 0 otherwise. The geometric features remain unchanged. The grounding for a pair of bounding boxes $\langle b_1, b_2 \rangle$ is the concatenation of the groundings of the single bounding boxes $\langle \bv_{b_1}: \bv_{b_2} \rangle$. However, when dealing with $n$-tuples of objects, adding some extra features regarding geometrical joint properties of these $n$ bounding boxes improves the performance of the LTNs model. Differently from \cite{donadello2017ijcai}, we add more joint features\footnote{All the features are normalized in the interval $[-1, 1]$.} that better capture the geometric interactions between bounding boxes:
\begin{multline}
\label{eq:grCC}
\bv_{b_1, b_2} = \langle \bv_{b_1}: \bv_{b_2}, ir(b_1, b_2), ir(b_2, b_1), \frac{area(b_1)}{area(b_2)}, \\ \frac{area(b_2)}{area(b_1)}, euclid\_dist(b_1, b_2), sin(b_1, b_2), cos(b_1, b_2) \rangle
\end{multline}
where:
\begin{itemize}
\item $\ir(b_1, b_2) = intersec(b_1, b_2)/area(b_1)$ is the inclusion ratio, see \cite{donadello2017ijcai};
\item $area(b)$ is the area of $b$;
\item $intersec(b_1, b_2)$ is the area of the intersection of $b_1, b_2$;
\item $euclid\_dist(b_1, b_2)$ is the Euclidean distance between the centroids of bounding boxes $b_1, b_2$;
\item $sin(b_1, b_2)$ and $cos(b_1, b_2)$ are the sine and cosine of the angle between the centroids of $b_1$ and $b_2$ computed in a counter-clockwise manner.
\end{itemize}
Regarding the \textbf{unary predicates} in $\P_1$, we adopt a rule-based grounding. Given a bounding box constant $b$, its feature vector $\bv_b=\left<v_1,\dots,v_{|\Pr_1|+4}\right>$, and a predicate symbol $C_i\in\Pr_1$, the grounding for $C_i$ is:
\begin{align}
\label{eq:grUnHot}
\pgsii(C_i)(\bv_b)=\left\{
\begin{array}{ll}
1 & \mbox{if } i = \argmax_{1 \leq l \leq |\Pr_1|}\bv_b^l \\ 
0 & \mbox{otherwise}.
\end{array}
\right. 
\end{align}
Regarding the \textbf{binary predicates} in $\P_2$, a rule-based grounding can be difficult to define as it requires a different analysis for each relation and could be inaccurate. Therefore, this grounding is learnt data by maximizing the truth values of the logic formulas in $\ksii$. The grounding of the \textbf{logical constraints} in $\ksii$ is determined by (i) instantiating a tractable sample of the constraints with the bounding box constants belonging to the same picture. (ii) Computing the groundings of the atomic formulas for every instantiated constraint; (iii) combining the groundings of the atomic formulas according to the LTNs semantics; (iv) aggregating the groundings of every instantiated constraint according to the LTNs semantics for universal quantification.

\subsection{The Optimization of $\gtsii$}
\label{sec:opt_sii}
Equation \eqref{eq:ltn_loss} defines how to learn the LTNs parameters by maximizing the grounding of the conjunctions of the formulas in $\ksii$. Here we study some pitfalls that can arise when the optimization is performed with the main t-norms:
\begin{description}
\item[\L{}ukasiewicz t-norm] The satisfiability of $\ksii$ is given by: $\pgsii(\bigwedge_{\phi \in \ksii}\phi) = \max\{0, \sum_{\phi \in \ksii}\pgsii(\phi) - |\ksii| + 1\}$. Thus, the higher the number of formulas the higher their grounding should be to have a satisfiability value bigger than zero. However, even a small number of formulas in $\ksii$ with a low grounding value can lead the knowledge base satisfiability to zero.
\item[G\"odel t-norm] The satisfiability of $\ksii$ is the minimum of the groundings of all its formulas: $\pgsii(\bigwedge_{\phi \in \ksii}\phi) = \min\{\pgsii(\phi) | \phi \in \ksii \}$. Here the optimization process could get stuck in a local optimum. Indeed, a single axiom (or predicate) could be too difficult to learn, the optimizer tries to increase this value without any improvement and thus leaving out the other axioms (or predicates) from the optimization.
\item[Product t-norm] The satisfiability of $\ksii$ is the product of the groundings of all its formulas: $\pgsii(\bigwedge_{\phi \in \ksii}\phi) = \prod_{\phi \in \ksii}\pgsii(\phi)$. As $\ksii$ can have many formulas, the product of hundreds of groundings can result in a very small number and thus incurring in underflow problems.
\end{description}
Differently from \cite{donadello2017ijcai}, we provide another definition of knowledge base satisfiability. We use a mean operator in Equation \eqref{eq:ltn_loss} that returns a \emph{global satisfiability} of $\ksii$ thus avoiding the mentioned issues:
\begin{equation}
\label{eq:ltn_loss_sii}
\mbox{$\Theta^*=\argmax_{\Theta}mean_p\left(\pgsii(\phi|\Theta) | \phi \in \ksii \right) - \lambda\lVert\Theta\rVert_2^2$},
\end{equation}
with $p \in \mathbb{Z}$. Here, we avoid values for $p$ bigger or equal than 1 as the obtained means are more influenced by the higher grounding values, that is, by the predicates ``easy'' to learn. These means return a too optimistic value of the satisfiability and this wrongly avoids the need of optimization. The computation of Equation \eqref{eq:ltn_loss_sii} is linear with respect to the number of formulas in $\ksii$.

\subsection{Post Processing}
Given a trained grounded theory $\gtsii$, we compute the set of groundings $\{\pgsii(\mathsf{r}(b,b'))\}_{\mathsf{r} \in \P_2}$, with $\langle b, b' \rangle$ a new pair of bounding boxes. Then, every grounding $\pgsii(\mathsf{r}(b,b'))$ is multiplied with a prior: the frequency of the predicate $\mathsf{r}$ in the training set. In addition, we exploit some equivalences between the binary predicates (e.g., beside is equivalent to next to) to normalize some groundings. In the specific, $\pgsii(\mathsf{r_1}(b,b')) = \pgsii(\mathsf{r_2}(b,b')) = \max\{\pgsii(\mathsf{r_1}(b,b')), \pgsii(\mathsf{r_2}(b,b'))\}$, if $\mathsf{r_1}$ and $\mathsf{r_2}$ are equivalent.

==> img/related_work.tex <==
\section{Related Work}
\label{sec:related-work}
The detection of visual relationships in images is tightly connected to Semantic Image Interpretation (SII) \cite{neumann2008onscene}. SII extracts a graph \cite{krishna2016visualgenome} that describes an image semantic content: nodes are objects and attributes, edges are relations between nodes. In \cite{neumann2008onscene} the SII graph (i.e., the visual relationships) is generated with deductive reasoning and the low-level image features are encoded in a knowledge base. Some logical axioms connect semantic classes of objects to their features. The work in \cite{Peraldi2009formalizing} uses abductive reasoning. However, writing axioms that map features into concepts/relations or defining the rules of abduction requires a high engineering effort, and dealing with the noise of the object detectors could be problematic. Fuzzy logic \cite{hajek2001metamathematics} deals with this noise. In \cite{Hudelot2008Fuzzy,Hudelot2014FCA} a fuzzy logic ontology of spatial relations and an algorithm (based on morphological and logical reasoning) for building SII graphs are proposed. These works are limited to spatial relations. In \cite{xu2017sceneGraph} the SII graph is built with an iterative message passing algorithm where the information about the objects maximizes the likelihood of the relationships and vice versa. LTNs have already been exploited for SII \cite{serafini2017learning,donadello2017ijcai}. These works are preliminary and focus only on the part-whole relation. Moreover, the experiments are conducted on a fully annotated dataset \cite{chen14PascalPart}.

Other methods start from a fully connected graph whose nodes and edges need to be labelled or discarded according to an energy minimization function. In \cite{kulkarni2011baby} the graph is encoded with a Conditional Random Field (CRF) and potentials are defined by combining the object detection score with geometric relations between objects and text priors on the types of objects. Also in \cite{chen14PascalPart} the scene graph is encoded with a CRF and the work leverages the part-whole relation to improve the object detection. These works do not consider logical knowledge. In \cite{chen2012understanding} the energy function combines visual information of the objects with logical constraints. However, this integration is hand-crafted and thus difficult to extend to other types of constraints.

A \emph{visual phrase} \cite{sadeghi2011recognition} is the prototype of a visual relationship. Here a single bounding box contains both subject and object. However, training an object detector for every possible triple affects the scalability. The \emph{visual semantic role labelling} \cite{gupta2015visual} is a generalization of detecting visual relationships. This task generates a set of tuples, such as: $\langle predicate, \{\langle role_1, label_1 \rangle, \ldots, \langle role_N, label_N\rangle\}\rangle$, where the roles are entities involved in the predicate, such as, subject, object, tool or place. However, the work is preliminary and limits the role of subject only to people.

Other works exploit deep learning. In \cite{Dai2017Detecting} the visual relationships are detected with a Deep Relational Network that exploits the statistical dependencies between relationships and the subjects/objects. In \cite{Liang2017Deep} a deep reinforcement learning framework to detect relationships and attributes is used. In \cite{Li2017ViP} a message passing algorithm is developed to share information about the subject, object and predicate among neural networks. In \cite{Zhang2017VtransE} the visual relationship is the translating vector of the subject towards the object in an embedding space. In \cite{yin2018zoom} an end-to-end system exploits the interaction of visual and geometric features of the subject, object and predicate. The end-to-end system in \cite{Zhang2017PPR-FCN} exploits weakly supervised learning (i.e., the supervision is at image level). LTNs exploit the combination of the visual/geometric features of the subject/object with additional background knowledge.

Background knowledge is also exploited in a joint embedding with visual knowledge. In \cite{ramanathan2015learning} the exploited logical constraints are implication, mutual exclusivity and type-of. In \cite{lu2016visual} the background knowledge is a word embedding of the subject/object labels. The visual knowledge consists in the features of the union of the subject and object bounding boxes. In \cite{tresp2017improvingVRD} the background knowledge is statistical information (learnt with statistical link prediction methods \cite{nickel2016Review}) about the training set triples. Contextual information between objects is used also in \cite{Zhuang2017context,Peyre2017Weakly} with different learning methods. In \cite{yu17vrd} the background knowledge (from the training set and Wikipedia) is a probability distribution of a relationship given the subject/object. This knowledge drives the learning of visual relationships. These works do not exploit any type of logical constraints as LTNs do.

